How Secure Are Large Language Models (LLMs) for Navigation in Urban Environments?

In the field of robotics and automation, navigation systems based on Large Language Models (LLMs) have recently demonstrated impressive performance. However, the security aspects of these systems have received relatively less attention. This paper pioneers the exploration of vulnerabilities in LLM-based navigation models in urban outdoor environments, a critical area given the widespread application of this technology in autonomous driving, logistics, and emergency services. Specifically, we introduce a novel Navigational Prompt Attack that manipulates LLM-based navigation models by perturbing the original navigational prompt, leading to incorrect actions. Based on the method of perturbation, our attacks are divided into two types: Navigational Prompt Insert (NPI) Attack and Navigational Prompt Swap (NPS) Attack. We conducted comprehensive experiments on an LLM-based navigation model that employs various LLMs for reasoning. Our results, derived from the Touchdown and Map2Seq street-view datasets under both few-shot learning and fine-tuning configurations, demonstrate notable performance declines across seven metrics in the face of both white-box and black-box attacks. Moreover, our attacks can be easily extended to other LLM-based navigation models with similarly effective results. These findings highlight the generalizability and transferability of the proposed attack, emphasizing the need for enhanced security in LLM-based navigation systems. As an initial countermeasure, we propose the Navigational Prompt Engineering (NPE) Defense strategy, which concentrates on navigation-relevant keywords to reduce the impact of adversarial attacks. While initial findings indicate that this strategy enhances navigational safety, there remains a critical need for the wider research community to develop stronger defense methods to effectively tackle the real-world challenges faced by these systems.

==> sections/0-title-author-abstract.tex <==
\title{How Secure Are Large Language Models (LLMs) for Navigation in Urban Environments?}

% \title{How Secure Are LLMs for Navigation in Urban Scenes?}
% You will get a Paper-ID when submitting a pdf file to the conference system
\author{Author Names Omitted for Anonymous Review. Paper-ID [416]}

%\author{\authorblockN{Michael Shell}
%\authorblockA{School of Electrical and\\Computer Engineering\\
%Georgia Institute of Technology\\
%Atlanta, Georgia 30332--0250\\
%Email: mshell@ece.gatech.edu}
%\and
%\authorblockN{Homer Simpson}
%\authorblockA{Twentieth Century Fox\\
%Springfield, USA\\
%Email: homer@thesimpsons.com}
%\and
%\authorblockN{James Kirk\\ and Montgomery Scott}
%\authorblockA{Starfleet Academy\\
%San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212\\
%Fax: (888) 555--1212}}


% avoiding spaces at the end of the author lines is not a problem with
% conference papers because we don't use \thanks or \IEEEmembership


% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\authorblockN{Michael Shell\authorrefmark{1},
%Homer Simpson\authorrefmark{2},
%James Kirk\authorrefmark{3}, 
%Montgomery Scott\authorrefmark{3} and
%Eldon Tyrell\authorrefmark{4}}
%\authorblockA{\authorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: mshell@ece.gatech.edu}
%\authorblockA{\authorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\authorblockA{\authorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\authorblockA{\authorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}

\newcommand{\revise}[1]{\textcolor{black}{#1}}

\maketitle

\begin{abstract}
\revise{In the field of robotics and automation, navigation systems based on Large Language Models (LLMs) have recently demonstrated impressive performance. However, the security aspects of these systems have received relatively less attention. This paper pioneers the exploration of vulnerabilities in LLM-based navigation models in urban outdoor environments, a critical area given the widespread application of this technology in autonomous driving, logistics, and emergency services. Specifically, we introduce a novel Navigational Prompt Attack that manipulates LLM-based navigation models by perturbing the original navigational prompt, leading to incorrect actions. Based on the method of perturbation, our attacks are divided into two types: Navigational Prompt Insert (NPI) Attack and Navigational Prompt Swap (NPS) Attack. We conducted comprehensive experiments on an LLM-based navigation model that employs various LLMs for reasoning. Our results, derived from the Touchdown and Map2Seq street-view datasets under both few-shot learning and fine-tuning configurations, demonstrate notable performance declines across seven metrics in the face of both white-box and black-box attacks.Moreover, our attacks can be easily extended to other LLM-based navigation models with similarly effective results. These findings highlight the generalizability and transferability of the proposed attack, emphasizing the need for enhanced security in LLM-based navigation systems. As an initial countermeasure, we propose the Navigational Prompt Engineering (NPE) Defense strategy, which concentrates on navigation-relevant keywords to reduce the impact of adversarial suffixes. While initial findings indicate that this strategy enhances navigational safety, there remains a critical need for the wider research community to develop stronger defense methods to effectively tackle the real-world challenges faced by these systems.}
\end{abstract}

\IEEEpeerreviewmaketitle

==> sections/1-intro.tex <==
\section{Introduction}
Robot navigation technology, a pivotal component in the modern automation landscape, empowers robots to independently move and execute tasks in diverse environments. This technology has become an indispensable core element in various domains such as autonomous driving~\cite{cui2023drivellm}, warehouse logistics~\cite{kenk2019human}, household services~\cite{eirale2022human}, and emergency rescue operations~\cite{colas20133d}. With the advent of foundational models in natural language processing and computer vision, robot navigation has seen significant enhancements. Notably, large language models (LLMs)~\cite{de2023llmr} possess unique advantages in distilling vast amounts of unstructured data into actionable insights, understanding complex natural language commands, and making real-time decisions. Applying LLMs to robot navigation tasks enhances robots' reasoning and decision-making abilities, enabling more accurate processing and interpretation of real-time visual data, which is crucial for navigation in dynamic and unstructured environments.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/fig_intro3.png}
    \caption{Comparison of navigation results of the VELMA-RBL~\cite{schumann2023velma} model before and after simple modifications to the navigation instructions.}
    \label{fig:intro}
\end{figure}



Depending on the application context, existing works utilizing LLMs for robot navigation can be categorized into indoor and outdoor scenarios. Indoor navigation tasks~\cite{yu2023l3mvn,zhou2023navgpt,yu2023co} based on LLMs typically involve directing robots to locate specific objects using textual input. In contrast, outdoor navigation tasks~\cite{shah2023lm,cui2023drivellm,schumann2023velma} often entail guiding robots through a series of instructions, including landmarks, to reach designated destinations. Although these approaches have shown promising results, most indoor navigation research relies on simulator-generated scenes or faces constraints in scale and trajectory length~\cite{schumann2023velma}. Outdoor scenarios, especially in urban environments, present unique practical challenges due to their complexity and diversity. Therefore, this paper focuses mainly on outdoor navigation in urban environments.

However, previous works have concentrated on designing LLM-based navigation systems, primarily aimed at enhancing navigation performance under normal conditions. A critical aspect that has received comparatively less attention is the inherent vulnerability of these LLM-based navigation models to potential threats. Previous studies~\cite{meng2022adversarial} have already demonstrated that most deep learning models, while robust in standard environments, can be easily deceived or disrupted when faced with carefully crafted adversarial inputs. Moreover, recent research~\cite{shi2023large} has revealed that LLMs, despite their advanced capabilities in processing and interpreting complex inputs, are exceptionally sensitive to a wide range of input variations. This sensitivity can lead to unexpected and erroneous outcomes, especially when LLMs are used as the primary decision-making framework in navigation systems. The potential for adversarial attacks to exploit these vulnerabilities and compromise the integrity of LLM-based navigation systems cannot be overlooked and needs to be thoroughly explored.

\revise{
In this paper, we explore for the first time the vulnerabilities of LLM-based navigation models in outdoor urban environments\revise{, as shown in Figure \ref{fig:intro}.} Inspired by previous adversarial attack strategies, we introduce a novel Navigational Prompt Attack tailored to the LLM-based navigation model. This form of attack involves perturbing the original navigational prompt by deriving gradients from the LLM model, causing the navigation model to predict incorrect actions. Based on the method of perturbation, our attacks are divided into two types: Navigational Prompt Insert (NPI) Attack and Navigational Prompt Swap (NPS) Attack. To validate the effectiveness of the proposed attacks, we conducted experiments on several variants of the VELMA model~\cite{schumann2023velma}, which utilizes diverse LLMs for reasoning, in both few-shot learning and fine-tuning experimental configurations.  The results indicated a significant decline in model effectiveness, uniformly observed across a range of attack scenarios, including both white-box and black-box methods, as evidenced by seven distinct metrics on two real-world street view datasets, Touchdown and Map2Seq. Crucially, our findings reveal the \textbf{generalizability and transferability} of these attacks, where a suffix generated for one LLM can effectively compromise navigation models based on different LLMs. This underscores the need for heightened security considerations in LLM-based navigation models, particularly in real-world settings like urban environments, where potential risks abound. Addressing these vulnerabilities, therefore, becomes crucial to ensure the reliability and security of LLM-based navigation systems in real-world applications. Furthermore, in response to the reduced reasoning capabilities resulting from these attacks, we have developed a preliminary countermeasure known as the Navigational Prompt Engineering (NPE) Defense strategy. This approach directs the model's attention towards keywords crucial for navigation, aiming to lessen the effects of adversarial suffixes. Experimental results indicate that this defensive method can moderately offset the performance deterioration caused by such adversarial attacks.}

% With the advent of foundation models in natural language processing and computer vision, navigation systems have witnessed substantial enhancements. These models, as cited in foundational research \cite{xxx}, empower navigation systems with the ability to tackle tasks necessitating reasoning and decision-making capabilities. Researchers have leveraged these models to significantly improve the decision-making abilities of robots within navigation frameworks. By enabling robots to process and interpret real-time visual data more accurately, foundation models facilitate navigation in dynamic and unstructured environments, making autonomous systems not only safer but also more efficient and adaptable. Consequently, the integration of foundation models into navigation systems marks a leap forward in robotics, expanding the horizons for autonomous systems.

% Building on recent technological advancements, language model-guided navigation has emerged as a pivotal field with two principal areas of focus: indoor and outdoor navigation. The former is associated with navigating through relatively static environments, marked by consistent room layouts and object placements. Conversely, outdoor navigation presents a far more dynamic challenge, grappling with unpredictable elements such as changing weather conditions, moving vehicles, and the intermittent presence of pedestrians. These factors substantially increase the complexity of navigating outdoor environments. In this work, we delve deeply into the challenges posed by outdoor navigation, aiming to thoroughly examine and address the nuanced difficulties and variables that complicate movement through these ever-changing spaces.

% Transitioning from the identification of these challenges, it becomes evident that the vulnerabilities inherent in outdoor navigation systems constitute a crucial yet insufficiently explored area within the realm of autonomous navigation. Despite remarkable progress in navigation technology, the unpredictable nature and complexity of outdoor settings continue to pose significant threats to the systems' reliability and safety. Research endeavors like VELMA \cite{} represent initial steps towards understanding and mitigating these vulnerabilities. However, the scarcity of comprehensive studies in this area highlights a substantial gap in our knowledge and capabilities, underscoring the urgency for more focused research. This gap not only limits our understanding but also restricts the practical deployment of outdoor navigation technologies in real-world scenarios, emphasizing the critical need for advancements in this domain. 

% Navigational proficiency is a cornerstone of modern automation, underpinning the operational success of various autonomous systems, including robotics and self-driving vehicles. These systems rely on the capacity to interpret complex environments and execute tasks with precision—capabilities that are particulsarly vital in real-world applications. As such, navigation is not just about reaching a destination but also about doing so efficiently, safely, and in real-time, responding to the dynamism of real-world scenarios. In sectors as diverse as urban planning, logistics, and personal transportation, the integration of advanced navigation systems holds the promise of transformative improvements.

% The integration of Large Language Models (LLMs) into navigational frameworks has introduced a paradigm shift, particularly evident in the domain of robotics and autonomous vehicular technology. LLMs possess the unique advantage of distilling vast amounts of unstructured data into actionable insights, understanding complex natural language commands, and making decisions in real-time. This has been applied extensively to indoor navigation tasks, where controlled environments provide the perfect testing ground for these intelligent systems. However, the true test of their utility lies in outdoor navigation— a domain fraught with unpredictability and infinitely more complex than the relatively static indoor settings. The real-world applicability of these models, particularly in outdoor scenarios, is where their potential can be truly realized or found wanting.

% However, the robustness of LLMs when deployed in outdoor navigation tasks remains a largely uncharted territory. This gap in knowledge is concerning, given the LLMs' inherent vulnerability to adversarial attacks that could lead to significant misdirections or errors in task execution. In the context of outdoor navigation, where the stakes include not just efficiency but also the safety of property and life, such vulnerabilities are untenable. It is this intersection of high-stakes application and potential for exploitation that necessitates a closer examination of LLMs' resilience.

% In response to this critical need, our research provides a comprehensive analysis of the fragilities present in current LLM-based outdoor navigation systems. We begin by detailing a series of novel attack vectors that exploit these weaknesses, effectively demonstrating the urgency for enhanced security measures. Following this, we propose and evaluate a suite of defensive strategies, rooted in the principles of Navigational Prompt Engineering (NPE) Defense, aimed at fortifying these intelligent systems against such adversarial manipulations. Our findings not only illuminate the risks associated with deploying LLMs in navigation tasks but also propose actionable solutions to reinforce their operational integrity, thereby paving the way for safer, more reliable real-world applications.





==> sections/2-related_work.tex <==
\section{Related Work}

\subsection{Large Language Models for Navigation} 
Recently, large language models (LLMs) have shown robustness and effectiveness for various tasks and applications. One of the remarkable tasks that has drawn more attention is navigation. The integration of LLMs into navigation systems demonstrates a significant shift from structured indoor environments to more unpredictable outdoor settings. Previous works have already investigated how to apply LLMs to indoor navigation in simulation or real-world environments. Yu \etal~\cite{yu2023l3mvn} demonstrates the potential of LLMs to improve robotic indoor navigation, and the proposed framework is tested in both simulated and real-world environments. Co-NavGPT~\cite{yu2023co} uses LLMs for global planning and assigning exploration frontiers among robots in a multi-robot navigation problem. Zhou \etal~\cite{zhou2023navgpt} proposes NavGPT, a purely LLM-based instruction following a navigation agent, which performs a zero-shot sequential indoor action prediction for vision-and-language(VLN) navigation. Shah \etal~\cite{shah2023navigation} integrates LLms to improve indoor robotic navigation tasks by proposing a Language Frontier guide (LFC), which uses LLMs to create semantic heuristics for planning and the planning guides the robot to explore unexplored areas more effectively. Note that these works are mainly based on simulations in which either the computer-generated images are with a fixed set of displayable objects and textures, or are limited in scale and trajectory lengths. These works usually suffer sharp performance drops when testing in unseen environments~\cite{schumann2022analyzing}. \revise{The emphasis in navigation technology is increasingly shifting toward zero-shot navigation, which seeks to equip robots with the capability to explore environments without any prior knowledge. In this context, Shah et al. \cite{shah2023navigation} introduce a method called semantic guesswork, which employs a large language model (LLM) to predict promising exploration frontiers that are likely to contain target objects. Similarly, the ESC framework \cite{zhou2023esc} utilizes the commonsense reasoning capabilities of LLMs to transform semantic scenes into natural language descriptions, assisting the robot in determining the next exploration point. Additionally, Song et al. \cite{song2023llm} apply an LLM as a zero-shot/few-shot planner that generates a series of actions for the robot, which are subsequently refined through a closed-loop feedback mechanism. In addition to indoor navigation.} Outdoor navigation is more complicated due to the realistic and unpredictable elements of these environments. In outdoor navigation, landmarks are first extracted, and then new instructions with descriptions of related landmarks are provided. Then, LLMs are responsible for predicting the agent's next step. Our work focuses mainly on outdoor navigation. Schumann \etal~\cite{schumann2023velma} demonstrates the applicability of LLMs in real-world scenarios. The landmarks are first extracted using CLIP, and then the fine-tuned models based on Llama~\cite{touvron2023llama} are required to make decisions when a robot comes to intersections. Shah \etal~\cite{shah2023lm} proposes LM-Nav, where GPT-3~\cite{brown2020language} is used for outdoor navigation. ~\citet{cui2023drivellm} also proposes a decision-making framework that combines LLMs with autonomous driving systems, enabling commonsense reasoning and learning from mistakes through a cyber-physical feedback system.

% Most prior work has been conducted in indoor scenarios where best results were obtained for navigation on routes that are similar to the training routes, with sharp drops in performance when testing on unseen environments~\cite{schumann2022analyzing}.

% Later, they also updated with Co-NavGPT \cite{yu2023co}. In this framework, they have used the LLM for multi-robot navigation problems. The LLM is mainly responsible for global planning and allocating exploration frontiers among robots. 

% Zhou et al. \cite{zhou2023navgpt} has also proposed NavGPT, a purely LLM-based instruction following a navigation agent that performs zero-shot sequential indoor action prediction for vision-and-language(VLN) navigation. 

% Shah et al. \cite{shah2023navigation} has also integrated LLms for enhancing indoor robotic navigation tasks. They proposed a Language Frontier guide(LFC), which uses LLMs to create semantic heuristics for planning. Then, the planning will guide the robot to explore unexplored areas more effectively. 

% \Cong{These tasks are mostly based on simulations that either feature computer-generated images with a fixed set of displayable objects and textures, or are limited in scale and trajectory length. }

% \Cong{Most prior work has been conducted in indoor scenarios where best results were obtained for navigation on routes that are similar to the training routes, with sharp drops in performance when testing on unseen environments. https://aclanthology.org/2022.acl-long.518.pdf}


% Transitioning to outdoor navigation tasks, the research becomes more intricate due to the realistic and unpredictable elements of these environments. In this category, landmarks are generally extracted first, and then new instructions also involve the description of the related landmark. Then, the LLM is responsible for predicting the agent's next step. Our paper is more focused on the outdoor navigation tasks. 

% For example, Schumann et al. \cite{schumann2023velma} has demonstrated the applicability of large language models used with real-world scenarios. They first extracted the landmarks using CLIP, then proposed fine-tuned models based on Llama and applied them to map2seq and touchdown datasets. LLMs are required to make decisions when it comes to intersections. 

% Shah\cite{shah2023lm} has proposed LM-Nav, where they used state of the art GPT-3 model for outdoor navigation tasks. In the work proposed by Cui et al. \cite{cui2023drivellm} authors have integrated LLMs into autonomous driving tasks, enabling commonsense reasoning in decision-making. This framework includes a cyber-physical feedback system for learning from mistakes, outperforming traditional methods in complex tasks. Beyond this, they have also demonstrated the robustness of LLM encountered with adversarial attacks.

\subsection{Security of Large Language Models}
With the expanding scope of LLM applications, their security has become a critical area of focus. Yao \etal~\cite{yao2023survey} categorizes LLM vulnerabilities into two categories: \textit{Inherent Vulnerabilities of the AI Model} and \textit{Vulnerabilities not Inherent to the AI Model}. The latter is unrelated to the LLM itself and usually requires a lot of extensive engineering tests to find such vulnerabilities. In contrast, inherent vulnerabilities can typically be detected through adversarial attacks. Wang \etal~\cite{wang2021towards} conducts an extensive survey on adversarial techniques to generate adversarial texts and designs the corresponding defense methods. Papernot \etal~\cite{papernot2017practical} introduces an adaptive black-box attack, and this method is further refined by Mahmood \etal~\cite{mahmood2021besting} which enhanced the attack and demonstrated $\geq30\%$ more effective than~\cite{papernot2017practical}. \revise{Zeng \etal~\cite{zeng2024johnny} proposes interpretable adversarial prompts to challenge AI safety for LLMs. A key difficulty in launching adversarial attacks on LLMs lies in the intrinsic discreteness of text, as opposed to the continuous nature of image input.}

This distinction makes it difficult to employ gradient-based optimization methods to effectively craft adversarial attacks. To solve such a problem, two solutions are suggested. One is embedding-based optimization, also known as soft prompting~\cite{lester2021power}, projects discrete tokens in some continuous embedding space. Unfortunately, the challenge is that the process is not reversible and LLMs usually do not allow users to provide continuous embeddings. The Prompts Made Easy (PEZ) algorithm~\cite{wen2023hard} solves these problems by using a quantized optimization that can project the result back into the hard prompt space. Another is one-hot encoding, which treats the one-hot vector as if it were a continuous quantity, as first proposed in HotFlip~\cite{ebrahimi2017hotflip}. However, the gradients at the one-hot encoding level may not provide an accurate representation of the function's behavior after an entire token is replaced. To solve the above problems, AutoPrompt~\cite{shin2020autoprompt} proposes a method based on gradient-guided search to automatically design prompts, which maximize the likelihood of prompting by constant iterative updating, and keep the prompt with the highest probability in the next step. Recently, ARCA~\cite{jones2023automatically} further improved this by evaluating not only the approximate one hot gradients at the original one-hot encoding of the current token, but also at several potential token swaps. \revise{More recently, Zou \cite{zou2023universal} proposed a method to jailbreak LLM using automatically generated adversarial suffixes.}

\revise{In addition to the adversarial attack method, it is important to design techniques to prevent the LLM from being fooled. Among the existing method, preprocessing input prompts using methods like perplexity filters \cite{jain2023baseline}, and paraphrasing \cite{jain2023baseline} have shown some effectiveness. Concurrent research also investigates heuristic detection-based methods, which have demonstrated strong performance in identifying adversarial inputs \cite{alon2023detecting}. Another innovative approach involves the use of safety filters on substrings of input prompts, offering certifiable robustness guarantees \cite{kumar2023certifying}. Although this method shows promise, its complexity scales with prompt length, posing a challenge for practical implementation. Robey\etal \cite{robey2023smoothllm} contributes to this body of work by developing a defense mechanism that perturbs input prompts at the character level, aggregating responses to detect and mitigate adversarial attacks.}

% “Vulnerabilities not inherent to the AI Model”, being unrelated to the LLM itself, usually need a lot of extensive engineering tests to be found. 


% While Inherent Vulnerabilities of the AI Models, which are directly connected to the model, typically can be detected through adversarial attacks. 

% Wang et al. \cite{wang2021towards} conducted an extensive survey on adversarial techniques for generating adversarial texts and the corresponding defense methods. Papernot et al. \cite{papernot2017practical} introduced the adaptive black-box attack toward machine learning. This method is further refined by Mahmood et al. \cite{mahmood2021besting} They have enhanced the attack and demonstrated $\geq30\%$ more effective than the original method. Zeng et al. \cite{zeng2024johnny} have proposed interpretable adversarial prompts to challenge AI safety for LLMs. 

% A key difficulty in deploying adversarial attacks on natural language processing (NLP) models lies in the intrinsic discreteness of text, as opposed to the continuous nature of image inputs. 

% This distinction makes it challenging to employ gradient-based optimization methods for crafting adversarial attacks effectively. To solve such a problem, people come up with two solutions. First, Embedding-based optimization, a technique often referred to as soft prompting \cite{lester2021power}, projects discrete tokens in some continuous embedding space. Unfortunately, the challenge is that the process is not reversible and large-scale languages do not allow users to provide continuous embeddings. The Prompts Made Easy (PEZ) algorithm solved these problems by using a quantized optimization, which can project the result back into the hard prompt space. 

% Second, one-hot encoding: which treats the one-hot vector as if it were a continuous quantity, and first used in HotFlip\cite{ebrahimi2017hotflip}. However, the gradients at the one-hot encoding level may not provide an accurate representation of the function's behavior after an entire token is replaced. In order to solve the above problems, AutoPrompt\cite{shin2020autoprompt} proposed a method based on gradient-guided search to automatically design prompts, which maximize prompt likelihood by constant iterative updating, and keep the prompt with the highest probability in the next step. Recently The ARCA method\cite{jones2023automatically} further improved this by not only eva;uating the approximate one-hot gradients at the original one-hot encoding of the current token, but also at several potential token swaps.


\subsection{Prompt Engineering Technique}
% The use of large language models as a replacement for supervised learning was popularized by the GPT series of language models~\cite{radford2019language}. Prompting both in the zero-short and few-shot settings has been explored widely in NLP tasks~\cite{gao2021making,le2021many,schick2021s,wei2022chain}. We consider only the case of human-readable prompts to large models, which contrasts with methods such as prompt tuning~\cite{lester2021power,li2021prefix}, which learns a continuous prompt embedding, and auto-prompting~\cite{shin2020autoprompt}, which attempts to search for prompts from scratch, both of which require a training step. For more examples see a recent survey by Liu \etal~\cite{liu2023pre}.

% The flexibility and effectiveness of prompt-based approaches encourage the use of prompting as the preferred way to interact with powerful NLP models. Writing good prompts to extract the desired information from a model is usually left to trial and error by the user, with few exceptions. 

% PromptSource~\cite{bach2022promptsource} increases the power of the templating language used to write general prompts. It also provides a platform for the community to create, evaluate, and explore new prompts.

% With the rapid development of large language models~\cite{brown2020language,ouyang2022training}, prompt engineering~\cite{gao2021making,schick2021s,weng2023towards} has become a promising paradigm for interacting with models~\cite{lester2021power}.

% With this paradigm, users can focus on designing and refining the prompt input to improve the performance of the pre-trained model in specific application scenarios, directly utilizing the knowledge and capability of the pre-trained model without the additional training process. 

% Gao \etal~\cite{gao2021making} employed the generative T5 model to generate the prompt templates and pruned brute-force search for label word selection.

% PromptIDE~\cite{strobelt2022interactive} provides interactive visualizations to help users
% evaluate the performance of prompts on a small dataset and iteratively
% refine prompts. For complex tasks that require multi-step operations,
% PromptChainer~\cite{wu2022promptchainer} allows users to interactively construct chains of
% prompts for the corresponding targeted sub-tasks, increasing the transparency and controllability of large language models.

With the release of the GPT series, the utilization of large language models as alternatives to supervised learning has acquired significant significance, as stated in~\cite{radford2019language}. Parallel to the rapid evolution of substantial large language models~\cite{brown2020language,ouyang2022training}, the engineering of prompts~\cite{gao2021making,schick2021s,weng2023towards} emerged as a prospective framework for model interactions~\cite{lester2021power}. By allowing users to focus on the design and refinement of prompt inputs, this framework makes it possible to improve the effectiveness of the pre-trained model in different applications. This is accomplished by directly utilizing the intrinsic knowledge stored in the pre-trained model, thereby avoiding any additional training phase. The application of prompt engineering has been widely studied~\cite{gao2021making,le2021many,schick2021s,wei2022chain}. This research has been conducted in both zero-shot and few-shot scenarios. There are three different types of prompting approach: the first is to use human-comprehensible prompts in large-scale models, and the second is to tune prompt, which involves learning a continuous prompt representation~\cite{lester2021power,li2021prefix}. The third type of prompting approach is auto-prompting~\cite{shin2020autoprompt}, which involves the autonomous generation of prompts from the ground up. Both of the latter two approaches require a phase of training. In the first type of prompting strategy, the user is often responsible for the work of developing efficient prompts to extract certain information from a model. This task frequently involves a trailing and error process. For the second and third prompt approaches, PromptSource~\cite{bach2022promptsource} enhances the capabilities of the templating syntax utilized in the formulation of generic prompts. More specifically, it provides a platform for the communal development, evaluation, and discovery of new prompts. Using the generative features of the T5 model \cite{raffel2020exploring}, Gao \etal~\cite{gao2021making} constructs prompt templates and accelerates the exhaustive search process to choose the label words. PromptIDE~\cite{strobelt2022interactive} offers users the opportunity to utilize interactive visual tools that assist them in evaluating the success of prompts within a small dataset and improve the cyclical functioning of the prompts. To improve the transparency and manageability of large language models, PromptChainer~\cite{wu2022promptchainer} enables users to constructively compose sequences of prompts that are suitable for specific subtasks. This is particularly useful for complex tasks that need multi-phased operations. There are more examples that can be found in a recent review by Liu \etal~\cite{liu2023pre}. Recent research also demonstrates that LLMs can also work as decent zero-shot reasoners~\cite{kojima2022large} by being prompted using a chain of prompts to endow LLMs with reasoning ability~\cite{wang2023plan,kong2023better}.

==> sections/3-attack.tex <==
\section{Vulnerabilities in LLMs for Navigation}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/fig_attack3.png}
    \caption{Illustration of the Navigational Prompt Suffix Attack. This approach involves attacking a specific LLM to identify an Adversarial Prompt Suffix. When this suffix is directly appended to a navigation prompt, it causes navigation systems based on that LLM, or other LLM models, to predict incorrect actions.}
    \label{fig:pipe}
\end{figure*}

\subsection{LLMs-based Navigation} \label{sec:llm_nav}

\subsubsection{Problem Statement} 
The primary goal of the navigation task is for the robot to determine the target location \( G \) from an initial state \( s_0 \), utilizing a set of navigation instructions denoted as \( n = (w_1, w_2, \ldots, w_N) \). In this undertaking, the robot must calculate a route that passes through a series of waypoints \( (\hat{v}_1, \hat{v}_2, \ldots, \hat{v}_T) \). The robot's state, signified as \( s = (v, \alpha) \), is characterized by its current position \( v \) among the network of nodes \( V \), and its orientation \( \alpha \). From the starting state \( s_0 \), the robot deduces the most likely next position by interpreting the navigation instructions \( w_i \) alongside the current observations \( o_i \), which encompass a panoramic view and the count of outward paths from its current node. The likelihood of the robot moving to the next position \( v_{t+1} \) is modeled by the following equation:
\begin{equation}
    v_{t+1} = \arg \max_{\bar{v} \in \bar{V}} P_{LLM}(\bar{v} | w_t, o_t)
    \label{eq:position_pred}
\end{equation}
where \( v_{t+1} \) represents the predicted next waypoint the robot aims to reach, \( \bar{V} \) is the set of all possible waypoints the robot can move to, \( w_t \) are the navigation instructions at time \( t \), and \( o_t \) are the observations at time \( t \). The function \( P_{LLM} \) provides the probability of reaching any given waypoint \( \bar{v} \) based on the current instructions and observations. The robot selects the waypoint with the highest probability as its next position.

Upon executing a move to the new position, the environment updates accordingly and transitions the robot into the subsequent state. This cycle of movement and transition continues iteratively. The robot progresses through this loop, advancing toward the designated goal, until it reaches a state where it predicts \( \act{stop} \), indicating that it has presumably arrived at the destination. The navigation task is considered successfully concluded when the robot's calculated position coincides with the target location \( G \), satisfying the navigational objective.


\subsubsection{Target Model \textbf{VELMA}} 

Translating this general framework into practical applications, we turn our attention to a specific example in the realm of LLM-based navigation. After a thorough analysis of existing navigation methods based on LLMs, we have selected {VELMA} as our target model due to its experiment settings that closely align with real-world environments. Unlike previous studies that were mainly focused on simulation environments or confined indoor spaces, VELMA is dedicated to exploring navigation tasks in actual city streetscapes, utilizing datasets such as {Touchdown} and {Map2seq}. This model demonstrates the efficacy of LLMs in long-distance navigation across real urban road networks and complex street scenarios. Therefore, we believe that hastily applying such navigation systems to the real world without a comprehensive analysis of their safety could lead to significant risks, particularly when taking into account the inherent vulnerabilities of deep learning models. Since LLMs are based on these neural network technologies, their unvetted deployment in real-world scenarios might trigger a series of societal problems and safety hazards.


% \noindent \paragraph{Problem Statement} 

As we introduced before, for the current navigation work based on LLMs, it essentially involves predicting the probability \( p(v_{i+1} | w_i, o_i) \) of the next position \( v_{i+1} \) based on the current navigation instruction \( w_i \) and observation \( o_i \). Specifically for VELMA, it has shifted the focus from predicting positions to predicting actions, where the action \( a \) is within the action space \( A \), defined as $A =\{\act{forward},\act{left},\act{right},\act{turn\_around},\act{stop}\}$. The formula for predicting the next action is expressed as:
\begin{equation}
    a_{t+1} = \arg \max_{\bar{a} \in A} P_{LLM}(\bar{a} | x_t),
    \label{eq:action_pred2}
\end{equation}
where $x_t$ represents the complete text prompt used as the input for the LLM at the current time \( t \). It is constructed by concatenating the task description \( d \), the navigation instructions text \( n \), followed by a sequence of observations \( o_i \), timestamps \( i \), and actions \( a_i \) for each timestep up to \( t-1 \), and finally appending the current observation \( o_t \) and the current timestamp \( t \). The formulation is as follows:
\begin{equation}
    x_t = [d, n] \oplus \bigoplus_{i=1}^{t-1} [o_i, i, a_i] \oplus [o_t, t],
    \label{eq:prompt3}
\end{equation}

% \noindent \paragraph{Methods} 

In the VELMA model, the first step involves the Landmark Extractor Module, which leverages LLM technology to derive a sequence of landmarks $(l_1, l_2, \ldots, l_L)$ from the given navigation instructions $n$. This is followed by the utilization of the Landmark Scorer Module, integrating CLIP, to evaluate whether each landmark $l_i$ is visible in the corresponding observation $o_i$. The next phase involves the Verbalizer Module, a template-based component, which produces textual descriptions of the environmental observations. These descriptions are subsequently integrated into the comprehensive prompt $x_t$. The model then proceeds to predict the subsequent action \(a_{t+1}\) by using the prompt \(x_t\) as input for the LLM, \revise{as delineated in Eq.~\ref{eq:action_pred2}.} The navigation task is considered complete when the model predicts the action \(\act{stop}\), indicating the robot considers itself to have reached the goal destination $g$.




\subsection{Navigational Prompt Attack}\label{sec:llm_attack}
As discussed in the previous section, LLMs are commonly utilized to predict the next location or action in navigation tasks, based on current instructions and observations. It is vital to ensure that these models produce reasonable and reliable outcomes. Nevertheless, the security and reliability aspects of existing LLMs, especially in the context of real-world navigation tasks, are not sufficiently explored.

In the realm of deep learning, particularly in image recognition, adversarial attacks often revolve around finding minute input data variations that can mislead the model. These variations are identified through the model's gradient. Attackers calculate the gradient of the model's output relative to the input data to craft subtle, nearly undetectable perturbations. When applied to the original input, these perturbations can cause the model to make erroneous predictions or classifications. \revise{Drawing inspiration from this methodology and related research, we have introduced two adversarial attack strategies for the LLM reasoning module used in robotic navigation tasks: \textbf{Navigational Prompt Insert (NPI) Attack} and \textbf{Navigational Prompt Swap (NPS) Attack}. These involve modifying the original prompt through insertion or swapping operations, respectively, to mislead the robot, causing it to generate incorrect location and action predictions. Our experiments show that these methods of perturbing the prompt are not only effective against specific target LLMs but also against other LLMs. This finding underscores the general applicability of such attacks. More importantly, it highlights the vulnerability of current LLMs in navigation scenarios, emphasizing the urgent need for the research community to focus more on the security aspects of deploying LLMs in real-world environments.}

% \revise{The main workflow of our method is illustrated in Figure \ref{fig:pipe}.} This strategy involves appending a specially crafted suffix to the complete prompt $x_n$ to lead the robot astray, making it generate incorrect location and action predictions. Our experiments demonstrate that this tailored suffix is not only effective against the specific target LLM but also proves to be potent for other LLMs. This finding underscores the general applicability of such attacks. More critically, it highlights the vulnerabilities of current LLMs in navigation scenarios, emphasizing the urgent need for the research community to focus more on the safety aspects of deploying LLMs in real-world settings.
\revise{Specifically, the core of the navigational prompt attack} is to minimize the likelihood of the LLM making an accurate prediction for the next action by perturbating the original prompt. To quantify this, we define a loss function \( \mathcal{L} \) as follows:
\begin{equation}
    \mathcal{L}(x_t, a_t) = - \log P_{LLM}(a_t | x_t)
\end{equation}

This loss function measures the negative logarithm of the probability that the LLM will correctly predict the next action \( a_t \) given the prompt \( x_t \). The objective of navigational prompt  attack is then formalized by the following optimization problem:
\begin{equation} \color{blue}
    \min \mathcal{L}(\hat{x}_t, a_t),
    \label{eq:obj_attack}
\end{equation}
\revise{\noindent where \( \hat{x}_t \) represents the perturbated navigational prompt.  Depending on the type of perturbation, adversarial navigation prompts can be categorized into insertion and swapping methods. By optimizing this loss, two types of navigational attacks effectively decrease the LLM’s likelihood of making accurate predictions in navigation scenarios, thereby exposing the model’s vulnerabilities to such adversarial interventions.}
% \noindent where \( X \) represents the set of all possible adversarial suffixes, \( \oplus \) denotes the operation of concatenating the suffix to the prompt, and \( \bar{x} \) is the generated adversarial suffix. By optimizing this loss, NPS Attack effectively decreases the LLM’s likelihood of making accurate predictions in navigation scenarios, thereby exposing the model’s vulnerabilities to such adversarial interventions.

% \begin{equation}
%     \min_{\bar{x} \in X} \mathcal{L}(x_t \oplus \bar{x}, a_t),
%     \label{eq:obj_attack}
% \end{equation}

\subsubsection{\revise{\textbf{Navigational Prompt Insert Attack (NPI) Attack}}} NPI Attack is a strategy designed to append a carefully crafted suffix to the original navigation prompt \( x_t \). The objective of the NPI Attack can be formalized by the following optimization problem:
\begin{equation}
    \min_{\bar{x} \in X} \mathcal{L}(x_t \oplus \bar{x}, a_t),
    \label{eq:obj_attack}
\end{equation}
\noindent where \( X \) represents the set of all possible adversarial suffixes, \( \oplus \) denotes the operation of concatenating the suffix to the prompt, and \( \bar{x} \) is the generated adversarial suffix. 

Unlike attacks on continuous inputs as seen in image processing, the input in Eq.~\ref{eq:obj_attack} consists of discrete text tokens. To execute a discrete attack, previous works typically employed a method of swapping the token that maximally decreased the loss. Building on similar ideas from these works, we first generate initial prompt $\widetilde{x}$ by adding a set of suffix tokens and then identify several possible token substitutions of suffix tokens according to the $k$ largest negative gradients with respect to one-hot token indicators. The formulation is as:
\begin{equation}
\mathcal{X}_i := \mbox{Top-}k(-\nabla_{e_{\widetilde{x}_i}} \mathcal{L}(\widetilde{x})), i \in \mathcal{S}, \\
\label{eq:topk}
\end{equation}
\noindent where $\mathcal{S}$ denotes the indices of the adversarial suffix tokens. By iterating over the set $\mathcal{S}$, we compile an initial set $\mathcal{X}$ of potential token substitutions. From this set $\mathcal{X}$, we then randomly select a subset $\mathcal{X}_B$ of tokens as candidates for replacement. The final step entails selecting the optimal replacement token from the subset $\mathcal{X}_B$ that minimizes the loss function $\mathcal{L}$. This process is expressed as the following formula:
\begin{equation}
\bar{x} = \underset{\bar{x} \in \mathcal{X}_B}{\mathrm{argmin}}\, \mathcal{L}(x_t \oplus \bar{x}, a_t),
\end{equation}
\noindent where $\bar{x}$ represents the token that, when replaced in the prompt, yields the smallest value of the loss function $\mathcal{L}$, thereby identifying the most advantageous adversarial token replacement.

\subsubsection{\revise{\textbf{Navigational Prompt Swap Attack (NPS) Attack}}} \revise{Unlike the NPI Attack, which appends a suffix directly to the original prompt without altering it, we have devised an alternative strategy that involves replacing words in the original prompt. Specifically, we aim to replace a word in the original prompt to decrease the likelihood that the navigation model will output the correct action. This optimization process can be described as follows:}
\begin{equation} \color{blue}
    \min_{\bar{x} \in X} \mathcal{L}(x_t \otimes \bar{x}, a_t),
    \label{eq:obj_attack}
\end{equation}
\revise{where \( X \)  represents the set of all possible tokens in the vocabulary that can be swapped, \( \otimes \) symbolizes the operation of swapping tokens within the prompt, and \( \bar{x} \) is the token selected from the dictionary to be swapped with a word in the original prompt.}

\revise{In order to minimize the perturbation to the original prompt, we replace only one word in the original prompt. To ensure that the replacement is a more meaningful word, specifically one that contains more critical navigational information, we first calculate the importance of each word. To ensure that our attack method is broadly applicable, that is, effective for both black-box and white-box attacks, we use the gradient response of the navigation model as a measure of word importance. This means we select the word with the greatest gradient response to the navigation model as the word to be swapped. Let \( x_t \) represent the original navigation prompt consisting of words \( w_1, w_2, \dots, w_n \). Our goal is to identify and replace one word in \( x_t \) to minimize the accuracy of the navigation model's output. The process can be summarized through the following steps:}
\begin{enumerate} \color{blue}
    \item \textbf{Calculate Word Importance:}
    We compute the importance of each word \( w_i \) in the prompt based on the gradient response with respect to the model's output. This can be represented as:
    \[
    \text{Importance}(w_i) = \left\lvert \nabla_{w_i} \mathcal{L}(x_t, a_t) \right\rvert
    \]
    Here, \( \mathcal{L} \) is the loss function of the navigation model, \( a_t \) is the desired action or output from the model, and \( \nabla_{w_i} \mathcal{L} \) represents the gradient of the loss with respect to word \( w_i \).

    \item \textbf{Select the Word to Swap:}
    We identify the word \( w_i \) with the highest gradient magnitude as the word to replace. This is because a higher gradient magnitude indicates a higher sensitivity of the output to changes in this word:
    \[
    w_{\text{swap}} = \underset{w_i}{\mathrm{argmax}}\, \text{Importance}(w_i)
    \]

    \item \textbf{Word Replacement:}
    After identifying \( w_{\text{swap}} \), the original prompt \( x_t \) can be represented as: $ x_t = x_{t, \text{b}} \oplus w_{\text{swap}} \oplus x_{t, \text{a}} $, where \( x_{t, \text{b}} \) represents the sequence of words in \( x_t \) before \( w_{\text{swap}} \), and \( x_{t, \text{a}} \) represents the sequence of words in \( x_t \) after \( w_{\text{swap}} \). We then select a swap token \( \bar{x} \) from a dictionary \( X \) using an equation referred to as Eq.~\ref{eq:topk} to swap \( w_{\text{swap}} \). The swap process can be described using the optimization formula where \( \bar{x} \) minimizes the loss function:
    \[
    \bar{x} = \underset{\bar{x} \in X}{\mathrm{argmin}}\, \mathcal{L}(x_{t, \text{b}} \oplus ( w_{\text{swap}} \otimes \bar{x} ) \oplus x_{t, \text{a}}, a_t)
    \]
\end{enumerate}


% Unlike continuous inputs as seen in image processing, the input in Eq.~\ref{eq:obj_attack} consists of discrete text tokens. To conduct a discrete attack effectively, previous methods typically involve identifying the token that, when swapped, maximally decreases the loss. Building upon these methodologies, we first identify critical tokens in the original prompt \( \widetilde{x} \) that are susceptible to manipulation and then calculate the gradients with respect to their positions. The formula used is:
% \begin{equation}
% \mathcal{X}_i := \mbox{Top-}k(-\nabla_{e_{\widetilde{x}_i}} \mathcal{L}(\widetilde{x})), i \in \mathcal{I},
% \end{equation}
% where \( \mathcal{I} \) indicates the indices of the critical tokens. By iterating over the set \( \mathcal{I} \), we compile an initial set \( \mathcal{X} \) of potential token positions for swapping. From this set \( \mathcal{X} \), we then select a subset \( \mathcal{X}_B \) of positions as candidates for the swap. The final decision involves choosing the optimal token position from \( \mathcal{X}_B \) that minimizes the loss function \( \mathcal{L} \). This selection process is formulated as:
% \begin{equation}
% \bar{x} = \underset{\bar{x} \in \mathcal{X}_B}{\mathrm{argmin}}\, \mathcal{L}(x_t \otimes \bar{x}, a_t),
% \end{equation}
% where \( \bar{x} \) represents the position that, when swapped in the prompt, results in the lowest value of the loss function \( \mathcal{L} \), thus identifying the most effective adversarial token swap.


\subsection{Experiment for NPS Attack in LLMs-based Navigation}\label{sec:exp_res}

\subsubsection{Datasets} 
{\paragraph{\textbf{Touchdown}}: Touchdown: The touchdown dataset is proposed by \citet{chen2019touchdown}. This dataset is created based on the Google Street View of New York City. The touchdown dataset contains 9,326 examples of English instructions and spatial descriptions paired with demonstrations. Each position includes \revise{a 360\degree RGB panorama} and all the panoramas are connected in a graph-like structure with undirected edges connecting neighboring panoramas. The environment includes 29,641 panoramas and 61,319 edges in total. The process is split into four crowdsourcing tasks: instruction writing, target propagation to panoramas, validation, and segmentation. Here, the two main tasks are writing and following. During the writing stage, a leader follows a prescribed route and hides Touchdown Bear at the end while writing navigation instructions that describe the path. The following stage involves following the written navigation instructions from the same starting position to find the Touchdown but only showing panoramas without the map.

\paragraph{\textbf{Map2seq}} Map2Seq Dataset is originally proposed by \citet{schumann2020generating} based on OpenStreetMap(OSM). OSM is \revise{a set of geodata} that provides detailed street layouts and annotations such as amenities, infrastructure, or land use. Map2Seq Dataset exported an OSM extract of Manhattan in 2017 and discretized the street layout by creating a node every ten meters along the roads. Routes are then sampled with lengths between 35 and 45 nodes. Afterwards, they used Amazon Mechanical Turk(AMT) to acquire human annotators. The first annotator is shown a specific route mentioned above and asked to write navigation instructions, including visual landmarks, without seeing the true panorama images. Then, a different annotator validates navigation instructions by using them to follow the route in the panorama environment without the map. Eventually, the dataset contains 7,672 navigation instructions.

\input{tables/attack_results}

\subsubsection{Baseline Models}
\paragraph{\textbf{VELMA-GPT3}}
The reasoning LLM used in VELMA-GPT3 is the advanced GPT-3.5 Turbo, an enhanced version of the original GPT-3 framework proposed by ~\citet{brown2020language}, featuring 175 billion parameters. This model integrates refined techniques to augment reasoning and language understanding capabilities.

% \paragraph{\textbf{VELMA-GPT4}}
% In VELMA-GPT4, the reasoning LLM is OpenAI’s latest GPT-4 Turbo, boasting 1.7 trillion parameters. As documented by Achiam, this model surpasses its predecessor GPT-4~\cite{achiam2023gpt} in efficiency, representing a significant leap in language processing technology.

% \paragraph{\textbf{VELMA-OPT}}
% The VELMA-OPT model utilizes the OPT (Open Pre-trained Transformer) as its reasoning language model. Developed by Meta AI and introduced by ~\citet{zhang2205opt}, OPT is designed to rival the performance of GPT-3 models. This family of transformer models offers a range of sizes; for our specific application, we have chosen the 1.3 billion parameter version. 

\paragraph{\textbf{VELMA-LLaMa}}
For VELMA-LLaMa, the reasoning LLM is Meta AI's LLaMa~\cite{touvron2023llama1}, which, unlike GPT-3, is trained solely on publicly available data. As demonstrated in the research, this 7 billion parameter model outperforms the GPT-3 model in several aspects.

\paragraph{\textbf{VELMA-LLaMa2}}
VELMA-LLaMa2 utilizes the second iteration of the original LLaMa model~\cite{touvron2023llama2} as its reasoning LLM, which features enhanced training and safety measures. The 7-billion parameter LLaMa-2 model demonstrates improved performance over its predecessor, especially in context understanding and data processing.

\paragraph{\textbf{VELMA-FT}}
The VELMA-FT model~\cite{schumann2023velma} incorporates a fine-tuned LLaMa-7b as its reasoning LLM. This fine-tuning process is specifically conducted on all training instances of the dataset, with each instance representing a complete text sequence developed from the most effective pathway. 

\paragraph{\textbf{VELMA-RBL}}
VELMA-RBL~\cite{schumann2023velma} employs the LLaMa-7b model as its reasoning LLM, integrating a response-based learning approach. This method enhances the learning process by combining actual data outcomes (ground truth data) with the model's generated outputs. The process employs a mixture of teacher and student forcing techniques, optimizing the model's ability to accurately interpret and respond to complex language queries, thereby improving its overall linguistic performance and adaptability in diverse scenarios.

\subsubsection{Evaluation Metrics}
\paragraph{\textbf{Shortest path distance (SPD)}} The SPD metric computes the minimal path length from the point where the agent ceases movement to the designated goal location.

\paragraph{\textbf{Key point accuracy (KPA)}} The KPA metric quantifies the percentage of accurate navigational choices made at key points. Such points encompass the starting point, intersection choices aligning with the optimal route, and the endpoint of the navigation.

\paragraph{\textbf{Task completion (TC)}} The TC metric is a binary metric evaluating whether the agent has achieved its navigation goal by stopping within the immediate proximity of the target node.
\revise{
\paragraph{\textbf{First Key Point Error (FKPE)}}
The FKPE metric evaluates the accuracy of navigation systems at the first key intersection points.}
\revise{
\paragraph{\textbf{Danger Impact (DI)}}
The DI metric assesses the potential risks associated with incorrect navigational decisions. This metric is focused on whether the agent stops at unsafe intersections.}
\revise{
\paragraph{\textbf{Path Length (PL)}}
The PL metric quantifies the total distance, measured as the number of nodes, from the start to the end of the route. 
}
\revise{
\paragraph{\textbf{Task Completion within 1 Node (TC-1)}}
The TC-1 metric is an extension of the standard TC metric. It evaluates whether the navigation system stops within one node of the target destination, thereby offering a more lenient criterion for success.
}

\subsubsection{\revise{{Implementation Details}}}

\revise{In our experiments, the VELMA model, configured with Llama-1 and Llama-2 as reasoning components, was subjected to local inference on a 80G A100 GPU in our local machine setup. Conversely, for models employing GPT-3 and GPT-4 as reasoning engines, inference processes were conducted remotely via the OpenAI API. Each navigation instance required up to 40 API calls. The expenses incurred for using GPT-3 and GPT-4 on the Touchdown dataset were approximately 105 dollars and 650 dollars respectively, while on the Map2seq dataset, the costs were about 120 dollars and 700 dollars respectively. These costs are subject to vary depending on actual usage conditions.}

\subsubsection{Results }

\paragraph{\textbf{Results for NPI Attack}} 
% Following the experimental setup in the original VELMA paper, we evaluated the results of two types of experiments: few-shot setting and fine-tuning setting. In the few-shot experiment, we conducted 2-shot in-context learning, randomly selecting two complete text sequences from the initial prompt training set navigational instances. For this task, we chose GPT-3, LLaMa1, and LLaMa2 as our reasoning models, none of which updated their weights. In the finetuning experiment, we finetuned VELMA-FT and VELMA-RBL, both based on LLaMa-7b, using all training instances of their respective datasets. In our experiments, we primarily generated suffixes based on two LLMs, LLaMa~\cite{touvron2023llama} and Vicuna~\cite{vicuna2023}, and applied these generated suffixes to the input prompt of aforementioned models. Depending on whether the suffix generated for the targeted LLM model is applied to the original LLM model or other LLM models, we categorized the attacks into white box attacks and black box attacks. That is, applying a suffix generated by LLaMa to a model using LLaMa for reasoning is considered a white box attack, while applying a suffix generated by LLaMa to models using other non-LLaMa LLMs is considered a black box attack. The same applies to suffixes generated by Vicuna.
\revise{Following the experimental setup in the original VELMA, we assessed two experimental setups: a few-shot and a fine-tuning setting. The few-shot experiment involved 2-shot in-context learning using GPT-3, LLaMa1, and LLaMa2 as static reasoning models, with two text sequences randomly selected from the training set. For the fine-tuning experiment, we adapted VELMA-FT and VELMA-RBL, both derived from LLaMa-7b, using their full datasets. We focused on generating suffixes using LLaMa \cite{touvron2023llama} and Vicuna \cite{vicuna2023}, which were then applied to the input prompts of the tested models. We distinguished between white-box NPI attacks, where suffixes are applied to the same LLM type as they were generated from, and black-box NPI attacks, which involve applying suffixes to different LLM types. Table \ref{tab:res_attack} presents the NPI results of VELMA models with GPT-3, LLaMa, and LLaMa2 as reasoners in 2-shot in-context learning, as well as VELMA-FT and VELMA-RBL in fine-tuning. The original results are unmarked, while results with suffixes from the NPS attack on LLaMa and Vicuna are denoted by $\dagger$ and $\ddagger$ respectively. White-box attacks are indicated by $\circ$, and black-box attacks by $\bullet$. We quantified the impact of attacks by calculating the percentage change in performance metrics post-attack, showing an increase in SPD (where lower is better) and a decrease in KPA and TC (where higher is better).}

% Table \ref{tab:res_attack} shows the NPI results of VELMA models with GPT-3, LLaMa, and LLaMa2 acting as reasoners in 2-shot in-context learning and the results of VELMA-FT and VELMA-RBL in finetuning. Unmarked results represent the original outcomes, $\dagger$ represents results with suffixes generated by the NPS attack applied to LLaMa in the input prompt, and $\ddagger$ represents the results with suffixes generated by the NPS attack applied to Vicuna in the input prompt. $\circ$ indicates white-box attacks, and $\bullet$ indicates black-box attacks. It is observed that adversarial prompt suffixes derived from different LLMs reduced navigational accuracy to some extent. To more clearly discern the effects before and after the attack, we calculated the percentage change of the post-attack values relative to the original values. For SPD, where lower values are better, our attack caused an increase. For KPA and TC, where higher values are preferable, our attack led to a decrease.

\textbf{White-Box Attacks}:
\revise{Table~\ref{tab:res_attack} highlights the vulnerabilities of both non-finetuned and finetuned VELMA models under adversarial NPS attacks. For non-finetuned models, VELMA-LLaMa and VELMA-LLaMa2, initial tests in 2-shot in-context learning displayed very low TC accuracies, i.e., under 4\%. When subjected to white box attacks, both models showed significant increases in SPD, i.e., up to 14.44\%, and sharp declines in KPA, i.e., up to 69.13\%, indicating their susceptibility to such attacks. In addition to the previously mentioned three metrics, we also assessed the attack's impact on four additional metrics within the Map2seq dataset. The outcomes are displayed in Table \ref{tab:I1}, where the $\circ$ symbols indicate the results. All metrics show significant deterioration post-attack compared to their values before the attack.}

\revise{The finetuned models, VELMA-FT and VELMA-RBL, while initially showing better performance, also experienced considerable performance degradation under attack. On the Touchdown and Map2seq datasets, both models underwent substantial increases in SPD (up to 85.26\%) and significant decreases in KPA and TC (up to 90.13\% in TC), demonstrating that even enhanced models are not immune to the effects of targeted adversarial prompts. This suggests a critical vulnerability in current LLM-based navigation models to simple suffix-based attacks.
Similarly, we have evaluated the impact of the black-box attack on the same four metrics. The results are presented in the row marked with $\bullet$ in Table \ref{tab:I1}.}
% As shown in Table~\ref{tab:res_attack}, the original VELMA-LLaMa and VELMA-LLaMa2, without undergoing training and being directly applied in 2-shot in-context learning, resulted in low TC accuracy in their navigational outcomes, with less than 4\% accuracy. Therefore, we primarily analyze the before-and-after comparison of VELMA-LLaMa and VELMA-LLaMa2 under attack based on the SPD and KPA metrics. By analyzing the values before and after the white box attack from the table, we can see that on the Touchdown dataset, VELMA-LLaMa and VELMA-LLaMa2 experienced an increase in SPD by 9.09\% and 4.65\% respectively, and a decrease in KPA by 69.13\% and 57.72\%. On the Map2seq dataset, VELMA-LLaMa and VELMA-LLaMa2 experienced an increase in SPD by 13.35\% and 14.44\% respectively, and a decrease in KPA by 43.67\% and 64.35\%. This shows that VELMA-LLaMa and VELMA-LLaMa2 are quite vulnerable and easily affected by this type of NPS attack.

% In the finetuning experiments, VELMA-FT and VELMA-RBL, having been finetuned, showed higher results across multiple metrics. Therefore, we analyzed the before-and-after comparison of VELMA-FT and VELMA-RBL under attack across the SPD, KPA, and TC metrics. On the Touchdown dataset, VELMA-FT and VELMA-RBL experienced an increase in SPD by 56.91\% and 85.26\% respectively, a decrease in KPA by 43.80\% and 71.14\%, and a decrease in TC by 62.26\% and 84.08\%. On the Map2seq dataset, VELMA-FT and VELMA-RBL experienced an increase in SPD by 259.38\% and 132.97\% respectively, a decrease in KPA by 64.67\% and 58.00\%, and a decrease in TC by 90.13\% and 73.18\%. It is evident that even for the finetuned models, our NPS attack can significantly decrease their navigational performance. This indicates that existing LLM-based navigation models are easily susceptible to attacks, which can be simply implemented by appending suffixes generated from attacking the LLMs to the input prompt.

\textbf{Black-Box Attacks}:
In the above section, we analyzed how suffixes generated by attacking the source LLM can significantly reduce the performance of navigation models that use the same LLM for reasoning. However, in practical application scenarios, we cannot know which LLM a navigation model is based on. Therefore, this section discusses whether suffixes generated by attacking other LLMs can impact navigation models that use different LLMs from the attacked ones.

\input{tables/attack_results_metric}

\revise{Analysis of VELMA-GPT3's performance on the Touchdown and Map2Seq datasets shows a marked decrease in navigational metrics after appending suffixes generated from attacks on LLaMa and Vicuna. On the Touchdown dataset, declines ranged from 19.82\% to 55.88\% across SPD, KPA, and TC metrics. Similarly, on the Map2Seq dataset, performance drops ranged from 11\% to 53\%. Suffixes from LLaMa attacks generally had a more detrimental impact than those from Vicuna. Additionally, VELMA-LLaMa and VELMA-LLaMa2, under black-box attacks in 2-shot context learning, showed KPA declines between 37\% and 64\%. For the finetuned models, VELMA-FT and VELMA-RBL, black-box attacks led to KPA and TC decreases ranging from 41\% to 72\%, confirming that adversarial prompts significantly impair navigational performance across various settings.}
% Firstly, by analyzing the navigational outcomes of VELMA-GPT3 with suffixes generated from attacking LLaMa and Vicuna added to the original navigation instructions, it is observed that suffixes generated by attacking two different LLMs can decrease the navigational performance of VELMA-GPT3 on the Touchdown dataset, with the navigation metric SPD, KPA, and TC dropping by 23.87\%, 49.49\%, and 55.88\%, as well as 19.82\%, 48.47\%, and 33.82\% respectively. Similarly, for the Map2Seq dataset, VELMA-GPT3's navigational performance across all three metrics dropped by 11\% to 53\% after the addition of suffixes generated from attacking two different LLMs. Among these, suffixes generated by attacking LLama had a greater impact on VELMA-GPT3 than those generated by attacking Vicuna. Similarly, by analyzing the results of VELMA-LLaMa and VELMA-LLaMa2 under black-box attacks in 2-shot context learning, we found a decline in these models' navigational performance. Notably, the accuracy of the KPA metric decreased by 37\% to 64\%. Additionally, for VELMA-FT and VELMA-RBL, which also underwent black-box attacks, the accuracy of the KPA metric decreased by 41\% to 53\%, and the accuracy of the TC metric decreased by 51\% to 72\%.

\revise{The experimental findings reveal a critical vulnerability in LLM-based navigation systems: their susceptibility to input perturbations, even those sourced from other LLMs. Notably, models like VELMA-GPT3, VELMA-LLaMa, VELMA-LLaMa2, VELMA-FT, and VELMA-RBL experience significant performance drops when exposed to such adversarial suffixes, highlighting the universal nature of this attack and the inherent fragility of LLMs. This suggests that these models may share underlying linguistic patterns or structures that are vulnerable to systematic manipulations. The differential impact of suffixes, notably more severe with those generated from attacking LLaMa compared to Vicuna, points to the influence of the source LLM's specific features—such as training data, architecture, or optimization strategies—on the attack's effectiveness. Understanding these factors is crucial for developing more robust LLM-based navigation systems.}

% The experimental results we have discussed highlight a significant vulnerability in LLM-based navigation systems: their sensitivity to perturbations in input prompts, even those generated by attacking other LLMs. Notably, models like VELMA-GPT3, VELMA-LLaMa, VELMA-LLaMa2, VELMA-FT, and VELMA-RBL demonstrate substantial performance declines, even when subjected to suffixes not derived from their foundational LLMs. This finding underscores the universality of our attack and the inherent fragility of current LLMs. It suggests these models may rely on similar underlying linguistic patterns or structures vulnerable to systematic manipulations. Furthermore, the more pronounced impact observed with suffixes generated from attacking LLama, as compared to Vicuna, points to the significant role played by the specific features of the source LLM in the effectiveness of the attack. This variation may be attributed to differences in training data, architectural design, or optimization strategies among LLMs. Recognizing these elements is critical for the future development of more resilient LLM-based navigation systems.

In summary, our experiments underscore the instability of current LLM-based models under attack, raising a cautionary note for the community regarding the application of LLM-based navigation in real-world scenarios. The vulnerabilities we have identified necessitate integrating adversarial training or other robustness-enhancing techniques in the development of LLM-based systems. Developers should focus not only on performance under standard test conditions but also on the resilience against increasingly complex and feasible adversarial manipulations. The subsequent sections will preliminarily propose defensive strategies against such attacks, providing initial insights for ongoing research.

\paragraph{\textbf{Results for NPS Attack}} 

\input{tables/attack_swap_results}

\revise{In this section, we report the results of our NPS Attack. Depending on the scenarios described in the prompts, our swap attacks can be categorized into attacks on intersections and landmarks. Table~\ref{tab:attack_swap_res} displays the results of the two types of NPS attacks for the VELMA-FT and VELMA-RBL models on both the Touchdown and Map2Seq datasets. $\dagger$ represents the results of attacks on prompts describing intersections, while $\ddagger$ indicates the results of attacks on prompts describing landmarks. The results demonstrate that our NPS attack are effective across both models on the two datasets. Particularly notable is the impact on the First Key Point Error (FKPE) metric, where the likelihood of the navigation agent making an error at the first intersection significantly increases. Furthermore, a comparison reveals that attacks on prompts describing intersections are more effective than those on prompts describing landmarks.}

\revise{\subsection{Discussion}}

\subsubsection{\revise{\textbf{NPI Attack in LM-Nav}}} \\

\input{tables/lmnav_attack}

\revise{
To further show that this vulnerability extends to other LLM-based navigation models, we applied our proposed NPI attack to another such model, LM-NAV\cite{shah2023lm}. LM-Nav is a robotic navigation system built entirely from pre-trained models for navigation (ViNG), image-language association (CLIP), and language modeling (GPT-3), eliminating the need for fine-tuning or language-annotated robot data. It includes three pre-trained models: a large language model (LLM) for extracting landmarks, a vision-and-language model (VLM) for grounding, and a visual navigation model (VNM) for execution. The effectiveness of the model was validated with 20 queries across two environments, totaling over 6km in combined length.}



\revise{
To investigate the LM-NAV model's vulnerability to NPI attacks, we appended the suffix generated by attacking the LlaMa model onto the LM-NAV model's input textual instructions. Following the experimental setup in LM-NAV, we evaluated the navigational performance after the attack in two experimental settings, EnvSmall-10 and EnvLarge-10. The results, as documented in Table~\ref{tab:LMnav}, reveal a decrease in the success rate from 0.8 to 0.1 (a decline of 87.50\%) in EnvSmall-10, and from 0.8 to 0.3 (a decline of 62.50\%) in the larger environment. To intuitively demonstrate the attack's impact, we plotted route maps before and after the attack, as depicted in Fig.~\ref{fig:lmnav}. The comparative route maps clearly illustrate significant differences in the LM-Nav model's navigation paths before and after the attack. After the attack, robots utilizing this model for navigation took substantially longer routes and failed to locate the target. This observation extends beyond a single LLM-based navigation system, highlighting a broader vulnerability. Consequently, this emphasizes the urgent need to address and focus on this issue, reinforcing the importance of understanding and mitigating vulnerabilities within LLM-based navigation systems to enhance their reliability and performance in real-world applications.
}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/fig_lmnav2.pdf}
    \caption{Comparative route map of the LM-Nav model's navigation results on a randomly selected route before and after the NPI attack.}
    \label{fig:lmnav}
\end{figure}}


% \subsubsection{\revise{\textbf{Results on Additional Metrics }}} \\


% \input{tables/1}
% \paragraph{\textbf{Shortest path distance (SPD)}} 

\subsubsection{\revise{\textbf{Comparison with Existing Attack Methods：}}} \\
\input{tables/2}
\revise{
In this section, we compare methods of adversarial suffix generation proposed in other domains to validate the advancement of our approach. Zou et al.~\cite{zou2023universal} introduced a novel class of adversarial attacks capable of inducing aligned language models to generate nearly any offensive content. We adapted this approach to serve as a baseline, tailoring it to better suit our navigation scenario requirements. We selected two models, VELMA-FT and VELMA-RBL, and compared their performance under both the baseline method and our attack strategy on the Map2Seq dataset. The results are listed in Table \ref{tab:attack_comparsion}. * denotes the baseline attack method, and $\dagger$ denotes our NPI attack method. It was found that our model is more effective than the baseline method, demonstrating the advanced nature of our attack technique.}
\revise{
This comparison not only highlights the relative effectiveness of our method but also underscores its utility in navigation-specific contexts. By showing superior performance on the Map2Seq dataset, we demonstrate that our method can effectively exploit vulnerabilities specific to navigation tasks, which are fundamentally different from the general content generation scenarios typically targeted by existing attacks.
}

\subsubsection{\revise{\textbf{Effect on insertion lengths of suffix}}} \\

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/I8_1.pdf}
    \caption{\revise{Impact of different insertion lengths on the performance of the NPI Attack.}}
    \label{fig:impact_suffix}
\end{figure}
\revise{
In this section, we explore the impact of different insertion lengths on the performance of the NPI Attack. Specifically, we used the VELMA-RBL model on the Map2Seq dataset to analyze how the model's performance metrics, including KPA, SPD, and TC, change as the percentage of inserted content increases. Figure~\ref{fig:impact_suffix}  displays the curves representing these changes. Initially, the metrics show little variation. However, as the insertion percentage reaches around 40\%, the curves for all three metrics sharply decline, leveling off when the insertion reaches approximately 80\%. This indicates that excessive insertion length is unnecessary and a certain threshold suffices to achieve effective adversarial impact.}

% \subsubsection{\revise{\textbf{Swap }}} \\
% % \input{tables/3}
% Google Doc, Item 7, Table

==> sections/4-defence.tex <==


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/fig_defense_diss.png}
    \caption{Examples of three Navigational Prompt Engineering (NPE) Defense strategies, NPE with Chain of Thought (NPE-Cot), NPE with Plan-and-Solve (NPE-PS), and NPE with Role-Play (NPE-RP), in a navigation instance.}
    \label{fig:defense_example}
\end{figure*}
\section{Enhancing Security in LLMs for Navigation}



\input{tables/defence_results_all}


In the previous section, we demonstrated that existing Large Language Models (LLMs) used for navigation reasoning are susceptible to attacks involving the addition of adversarial suffixes to the input prompt. This revelation compels us to address this vulnerability seriously. To explore potential strategies for mitigating the decline in reasoning capabilities caused by attacks on LLMs, this chapter discusses the use of prompt engineering as a method of defense. \revise{Difference method of defense is shown in Fig.~\ref{fig:defense_example}.} The motivation behind employing prompt engineering for defense primarily lies in the belief that by carefully designing prompts, we can direct the model's focus towards critical aspects of tasks or queries, thereby potentially neutralizing misleading or malicious inputs introduced by adversaries. This approach not only prevents external manipulation but also actively fosters a better understanding and handling of inputs by the model. With this concept in mind, we first propose the idea of Navigational Prompt Engineering (NPE) Defense in Section \ref{subsec:npe_defense}. Subsequently, in Section \ref{subsec:npe_defense}, we present experiments on NPE Defense in LLMs-based navigation tasks to verify its effectiveness against the aforementioned NPS attack.


\subsection{Navigational Prompt Engineering (NPE) Defense}
\label{subsec:npe_defense}

Prompt Engineering is an emerging technique in the field of artificial intelligence, particularly within the domain of LLMs. At its core, Prompt Engineering involves the strategic formulation of input prompts to guide the behavior of a language model. This practice is crucial in leveraging the full potential of LLMs, as the way a prompt is structured can significantly influence the model's output.

Given that the addition of suffixes generated by the NPS attack has been shown to diminish the reasoning capabilities of LLMs in navigation tasks, we propose a method called Navigational Prompt Engineering (NPE) Defense for LLM-based navigation tasks. This defense mechanism leverages the advantage of Prompt Engineering in enhancing the model's reasoning capabilities. The principle of this mechanism is to reinforce the LLM's interpretative abilities through carefully designed prompts. It focuses on reorganizing the input prompts to mitigate the impact of adversarial suffixes without the need to alter the underlying model training or architecture. The objective formulation is written by:

\begin{equation}
    a_{t+1} = \arg \max_{\bar{a} \in A} P_{LLM}(\bar{a} | f_{\text{NPE}} (x_t+\bar{x})),
    \label{eq:action_pred}
\end{equation}

\noindent where $\bar{x}$ is the generated adversarial suffix by attacking LLM based on NPS attack. $f_{\text{NPE}}$
is the function of NPE Defense to reorganize the input prompts.


\subsection{Experiment for NPE Defense in LLMs-Based Navigation}
\label{subsec:exp_defense}

\subsubsection{Experimental Setting}
In this section, we validate our proposed NPE Defense strategies in specific navigation experiments. Similarly, based on the navigation tasks of VELMA on the Touchdown and Map2seq datasets discussed in the previous section \ref{sec:exp_res}, we introduce adversarial prompt suffixes generated by attacking LLMs into the original navigation instructions as input for attacking various models. In this experiment, we selected three models from Table \ref{tab:res_attack}: VELMA-GPT3, VELMA-LLaMa2, and VELMA-RBL. Each of these models demonstrates strong initial navigational performance and represents a diverse range of types. For the NPS Attack method, we chose suffixes generated by attacking LLaMa, as it has stronger attack performance and can also represent both black box and white box attacks in this experiment. We base our defenses on three fundamental prompt engineering strategies, which are:

\paragraph{Zero-Shot Chain of Thought Prompting} Zero-shot-CoT~\cite{kojima2022large} regards LLMs as decent zero-shot
reasoners. To unleash the reasoning ability of LLMs, it adds a simple prompt, \ie, ``Let’s think step by step'', to facilitate step-by-step thinking before prompting each question to LLMs. Such a naive scheme could significantly improve the performance of LLMs in complex reasoning tasks without requiring task-specific examples. 

\paragraph{Plan-and-Solve Prompting} Though Zero-shot-CoT~\cite{kojima2022large} invokes LLMs' reasoning abilities by adding ``Let's think step by step'' to each prompt, yet it is still troubled by errors from calculation, missing-step, and semantic misunderstanding. To mitigate these issues, Plan-and-Solve (PS) Prompting~\cite{wang2023plan} proposes to divide tasks into subtasks for a systematic execution, and then derives PS+ prompting by adding detailed instructions, improving reasoning step quality and calculation accuracy.

\paragraph{Role-Play Prompting} LLMs like GPT-3.5~\cite{openai2023chatgpt} and GPT-4~\cite{openai2023gpt4} demonstrate profound role-playing abilities, extending beyond human personas to non-human entities. Kong \etal~\cite{kong2023better} further enhances LLMs' performance, particularly in zero-shot settings, with noticeable improvements in specific reasoning tasks, indicating that role-play prompting not only deepens contextual understanding but also acts as an implicit trigger for improved reasoning processes.

\subsubsection{Results}
For the sake of clarity in this discussion, the NPE defense methodologies derived from the three aforementioned strategies will henceforth be designated as NPE-CoT, NPE-PS, and NPE-RP, respectively. Table~\ref{tab:defence_all} presents a comparative analysis, encompassing the initial navigational results of the three specified target models, their performance subsequent to the NPS attack, and the outcomes following the implementation of each of the three distinct NPE defensive approaches on the models impacted by the attack.

As seen from Table~\ref{tab:defence_all}, in the 2-shot in-context learning experiments, the introduction of three types of NPE Defense strategies resulted in improvements across three metrics for both VELMA-GPT3 and VELMA-LlaMa2. In the fine-tuning experiments, the enhancements were even more pronounced with the VELMA-RBL model incorporating the three NPE Defense strategies. Notably, the NPE-RP defense strategy significantly increased VELMA-RBL's performance on the Touchdown dataset, with KPA rising from 14.9 to 32.0 (an increase of 114.77\%), and the TC metric from 3.9 to 12.8 (an increase of 228.21\%). Similarly, on the Map2seq dataset, KPA improved from 29.5 to 65.1 (an increase of 120.68\%), and the TC metric from 11.4 to 29.0 (an increase of 154.39\%).


\revise{\subsection{Discussion}}

\subsubsection{\revise{\textbf{Defense results on LM-Nav}}} \\
\revise{
In this section, we evaluate the defensive performance of our three proposed NPE strategies after the LM-NAV system has been subjected to attacks. We present results in Table~\ref{tab:defense_lmnav} that details the accuracy of the original LM-NAV, the accuracy after it has received an NPI attack, and the accuracy after the implementation of each of the three defense strategies, in two distinct environments: EnvSmall and EnvLarge. The results clearly demonstrate that all three of our defense strategies effectively mitigate the impact of the NPI attacks to varying degrees. Particularly, the defense performance in the EnvSmall environment is more robust. 
}
\input{tables/defense_lmnav}

\subsubsection{\revise{\textbf{Comparison of Different Defense Methods}}} \\
\revise{
In this section, we have additionally designed two defense methods to validate the effectiveness of our proposed defense strategies. First, we developed an adversarial training defense method, which involves retraining the model using the generated adversarial prompts and then testing its defensive performance on other unseen adversarial prompt samples. Additionally, we adapted the adaptive system prompt (ASP) method, a state-of-the-art defense strategy, proposed in \cite{zeng2024johnny} to suit our navigation scenario. We compared the results of these two methods along with our own NPE-RP defense strategy across two models, VELMA-FT and VELMA-RBL, on the Map2Seq dataset. The results are presented in Table \ref{tab:defense_ab}. The table reveals that the defense provided by adversarial training is limited. However, our defense method and the ASP method achieved comparable performance, which underscores the effectiveness and superiority of our proposed NPE strategies. This comparison demonstrates that our NPE approach is not only effective but also advantageous in enhancing the robustness of navigation systems against adversarial threats.}

\input{tables/5}  

\subsubsection{\revise{\textbf{Defense Performance When Adversarial Prompts Contain Meaningful Words}}} \\

\revise{
In this section, we examine the defensive performance of the model when our adversarial prompts contain tokens in the form of meaningful words mixed with random characters. To test this intriguing scenario, we evaluated the model's performance without any defense and compared it with the results obtained using three different defense strategies. We qualitatively present these results in Fig.~\ref{fig:defense_example}. As shown in the Fig.~\ref{fig:defense_example}, when input with such adversarial prompts, the model without any defense strategy directly outputs a "stop" action, whereas the models equipped with our defense strategies correctly output a "forward" action. This indicates that our defense methods are effective in discerning and mitigating the disruptive effects of adversarial prompts that blend meaningful content with noise.}

\revise{
The ability of our defensive strategies to maintain correct functionality under these conditions highlights their robustness and adaptability. This is particularly important in practical applications where adversarial inputs may not be purely disruptive but could mimic legitimate user commands interspersed with misleading information. The results suggest that our defensive approaches can effectively filter out the noise and focus on the meaningful elements of the prompts, ensuring that the navigation system remains reliable even in the face of sophisticated attacks. }
 
\subsubsection{\revise{\textbf{Defense Performance Under NPI Attacks with Different Insertion Positions}}}

\revise{In this section, we evaluate the effectiveness of our proposed NPE defense strategies under NPI attacks, which vary according to the insertion position of adversarial tokens. We specifically modified the NPI attack into three variants based on the location of the adversarial token insertion: at the start of the sentence (Insert\_S), in the middle of the sentence (Insert\_M), and at the end of the sentence (Insert\_E). We then assessed how the VELMA-RBL model performed on the Map2Seq dataset under these three types of NPI attacks.}

\revise{After applying our three proposed NPE defense strategies to each of these attack variants, we created a bar chart to visually represent the changes in navigation performance for each scenario, as illustrated in Fig.~\ref{fig:defense_vari_pos}. This visual comparison clearly shows the differential impact of each attack variant and the corresponding effectiveness of the applied defenses. The results indicate that our defense strategies effectively mitigate the effects of adversarial tokens regardless of their insertion points.  Moreover, the results suggest that the positioning of adversarial tokens can influence the effectiveness of the attack, and correspondingly, the efficacy of defense mechanisms. This analysis not only demonstrates the robustness of our defense strategies but also highlights their adaptability to different adversarial strategies
}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/test.pdf}
    \caption{\revise{
    Defense performance under NPI attacks with three different attack insertion positions: Insert-S (at the start of the sentence), Insert-M (in the middle of the sentence), and Insert-E (at the end of the sentence). The red bars represent the TC results without any attack. The bars immediately following depict the TC results with NPI attack. Subsequent groups of bars represent three defense strategies, including NPE-COT, NPE-PS, and NPE-RP.
    }}
    \label{fig:defense_vari_pos}
\end{figure}
% Google Doc, Item 11, Figure




==> sections/5-conclusion.tex <==
\section{Conclusion}
\revise{
In this study, we explore previously unexplored vulnerabilities of LLM-based navigation models in outdoor urban environments. We introduce novel attack methods, Navigational Prompt Insert (NPI) and Navigational Prompt Swap (NPS), demonstrating how perturbations to the original navigational prompt can mislead these models into making incorrect action predictions. Through comprehensive experiments involving various VELMA model variants and employing diverse LLMs under both few-shot learning and fine-tuning configurations, we observed a notable decrease in model effectiveness. This decline was consistent across a range of attack scenarios, including white-box and black-box methods, as evidenced by metrics on the Touchdown and Map2Seq street view datasets. Furthermore, our attacks are readily adaptable to other LLM-based navigation models, such as LM-Nav, achieving similar success. Our findings not only highlight the transferability of these attacks across different LLM-based navigation models but also underscore the urgent need for enhanced security measures in real-world applications. As an initial countermeasure, we propose the NPE Defense strategy, which focuses on navigation-relevant keywords to mitigate the impact of adversarial suffixes. Although preliminary results indicate that this strategy improves navigational safety, there remains a crucial need for the broader research community to develop more robust defense mechanisms to address the real-world challenges these systems face.}



\revise{
Regarding future research directions, we envisage several pivotal areas of focus that promise to advance the field of LLM-based navigation systems. Firstly, given the substantial resource consumption associated with large models, there is a critical need for research into lightweight network structures. Such structures would enable researchers with limited resources to efficiently run large models. This exploration could include developing more compact versions of existing architectures or innovating new methods to reduce computational demands without compromising performance. Secondly, the integration of multi-source data presents a significant research opportunity. Considering the availability of GNSS (Global Navigation Satellite System) in outdoor scenarios, combining these reliable location data with the contextual understanding capabilities of LLMs could enhance navigational accuracy and reliability. This direction involves exploring how different data types can be effectively synthesized to improve the decision-making processes of navigation models, especially in complex or obstructed environments where GNSS signals may be degraded. Thirdly, the development of more robust defense strategies is paramount. As adversarial attacks become more sophisticated, ensuring the security of LLM-based navigation systems is crucial. Future studies should focus on creating advanced defensive measures that can preemptively detect and mitigate potential threats. This includes exploring deeper layers of security protocols, enhancing adversarial training methods, and possibly employing artificial intelligence to dynamically adjust defensive mechanisms in response to detected threats.}


==> tables/attack_results_back.tex <==
\begin{table*}[h]
\centering
\caption{Results for the VELMA model with various LLM models before and after the Navigational Prompt Suffix Attack (NPSA) on the Touchdown and Map2seq datasets in the unseen scenario. \(\dagger\) represents the results after NPSA using the LLaMa suffix, and \(\ddagger\) represents the results after NPSA using the Vicuna suffix.}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
&\multicolumn{3}{c}{\textbf{Touchdown}} & \phantom{} &\multicolumn{3}{c}{\textbf{Map2seq}} \\ 
\cmidrule{2-4} \cmidrule{6-8} 
    \textbf{LLM Models} & \textbf{SPD\textdownarrow} & \textbf{KPA\textuparrow} & \textbf{TC\textuparrow} & \phantom{} & \textbf{SPD\textdownarrow} & \textbf{KPA\textuparrow} & \textbf{TC\textuparrow}\\
\toprule
&\multicolumn{6}{c}{\textbf{2-Shot In-Context Learning}}\\
\midrule
VELMA-GPT-3      & 22.2   & 49.1  & 6.8  && 19.1  &  58.1  &  9.2   \\
VELMA-GPT-3 \dagger      & 27.5   &  24.8  &  3.0  && 23.7  &  28.5  &  3.5   \\
VELMA-GPT-3 \ddagger      & 26.6  &  25.3  &  4.5  && 23.9  &  37.5  &  4.5   \\
\midrule
% VELMA-GPT-4      & {21.8}  & {56.1}  & {10.0}  && {12.8}  &  {70.1}  &  {23.1}   \\
% VELMA-GPT-4 \dagger      & -  &  -  &  -  && 18.2  &  63.7  &  14.0   \\
% VELMA-GPT-4 \ddagger      & -  &  -  &  -  && 16.6  &  65.5  &  16.4   \\
% \midrule
% VELMA-OPT      & 27.5  &  28.8  &  3.5  && 35.9  &  31.0  &  0.3   \\
% VELMA-OPT \dagger      & 26.6  &  28.2  &  2.5  && 36.6  &  30.0  &  0.1   \\
% VELMA-OPT \ddagger      & 29.3  &  28.3  &  1.9  && 36.7  &  30.5  &  0.1   \\
% \midrule
VELMA-LLaMa       & 35.2  &  44.7  &  1.3  && 35.2  &  44.5  &  1.4   \\
VELMA-LLaMa \dagger      & 38.4  &  13.8  &  0.4  && 39.9  &  16.9  &  0.1   \\
VELMA-LLaMa \ddagger      & 41.5  &  16.2  &  0.5  && 37.8  &  18.7  &  0.3   \\
\midrule
VELMA-LLaMa2     & 42.7  &  48.3  &  2.1  & & 35.7  &  57.7  &  3.2   \\
VELMA-LLaMa2 \dagger      & 45.0  &  15.6  &  0.5  & & 42.0  &  15.4  &  0.9   \\
VELMA-LLaMa2 \ddagger      & 44.3  &  16.3  &  0.7  & & 43.4  &  18.1  &  1.0   \\
\midrule
&\multicolumn{6}{c}{\textbf{LLM Finetuning, full training set}}\\
\midrule
VELMA-FT    & 18.3 & 62.0 & 23.4 && 8.7 & 78.7 & 41.3 \\
VELMA-FT \dagger    & 29.5 & 29.9 & 8.0 && 34.5 & 24.2 & 3.8\\
VELMA-FT \ddagger    & 25.4 & 30.2 & 10.3 && 22.4 & 38.5 & 15.6 \\
\midrule
VELMA-RBL     & 15.5 & 63.6 & 26.0&& 8.3 &  79.5 &  45.3 \\
VELMA-RBL \dagger    & 28.9 & 14.9 & 3.9 && 21.2 & 29.5 & 11.4 \\
VELMA-RBL \ddagger    & 21.0 & 32.5 & 11.2 && 27.0 & 32.5 & 11.5 \\
\bottomrule
\end{tabular}
}
\label{tab:results}
\end{table*}

==> tables/attack_results_metric.tex <==
\begin{table*}[h] 
\centering
\caption{Results for the VELMA-FT and VELMA-RBL model under FKPE, DI, PL and TC-1 metric before and after the Navigational Prompt Insert (NPI) Attack on the Touchdown and Map2seq datasets in the unseen scenario. $\dagger$ represents results with suffixes generated by the NPI attack applied to LLaMa in the input prompt, and $\ddagger$ represents the results with suffixes generated by the NPI attack applied to Vicuna in the input prompt. $\circ$ indicates white-box attacks, and $\bullet$ indicates black-box attacks.}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
% &\multicolumn{4}{c}{\textbf{Map2seq}} \\ 
% \cmidrule{2-5} 
    \textbf{LLM Models} & \textbf{FKPE\textdownarrow} & \textbf{DI\textdownarrow} & \textbf{PL\textdownarrow} & \textbf{TC-1\textuparrow} \\
\toprule
VELMA-FT      & 50   & 45  & 41  &  42.0   \\
\circ \text{VELMA-FT} \dagger        & 195 \scriptsize{(\textcolor{blue}{\textuparrow 290.00\%})}   & 70 \scriptsize{(\textcolor{blue}{\textuparrow 55.56\%})}  & 51 \scriptsize{(\textcolor{blue}{\textuparrow 24.39\%})}  &  9.1 \scriptsize{(\textcolor{red}{\textdownarrow 78.33\%})}   \\
\bullet \text{VELMA-FT} \ddagger      & 165\scriptsize{(\textcolor{blue}{\textuparrow 230.00\%})}   & 58\scriptsize{(\textcolor{blue}{\textuparrow 28.89\%})}  & 46\scriptsize{(\textcolor{blue}{\textuparrow 12.20\%})}  &  23.0\scriptsize{(\textcolor{red}{\textdownarrow 45.24\%})}   \\
\midrule
VELMA-RBL     & 47   & 30  & 42  &  44.5   \\
\circ \text{VELMA-RBL} \dagger      & 134\scriptsize{(\textcolor{blue}{\textuparrow 185.11\%})}   & 68\scriptsize{(\textcolor{blue}{\textuparrow 126.67\%})}   & 50\scriptsize{(\textcolor{blue}{\textuparrow 19.05\%})}   &  20.8\scriptsize{(\textcolor{red}{\textdownarrow 53.26\%})}    \\
\bullet \text{VELMA-RBL} \ddagger       & 107\scriptsize{(\textcolor{blue}{\textuparrow 127.66\%})}   & 56\scriptsize{(\textcolor{blue}{\textuparrow 86.67\%})}   & 45\scriptsize{(\textcolor{blue}{\textuparrow 7.14\%})}   &  24.4\scriptsize{(\textcolor{red}{\textdownarrow 45.17\%})}    \\
\bottomrule
\end{tabular}}
\label{tab:I1}
\end{table*}

==> tables/defence_results.tex <==
\begin{table*}[h]
\centering
\caption{Results for the VELMA model with various LLM models using three Navigational Prompt Engineering (NPE) Defense strategies after the Navigational Prompt Suffix (NPS) Attack on the Touchdown and Map2seq datasets in an unseen scenario. $\circ$ and $\bullet$ indicate white-box and black-box attacks, respectively, by applying the NPS Attack to the LLaMa model. NPE-Cot denotes NPE with Chain of Thought prompting, NPE-PS denotes NPE with Plan-and-Solve prompting, and NPE-RP denotes NPE with Role-Play prompting.
}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
&\multicolumn{3}{c}{\textbf{Touchdown}} & \phantom{} &\multicolumn{3}{c}{\textbf{Map2seq}} \\ 
\cmidrule{2-4} \cmidrule{6-8} 
    \textbf{LLM Models} & \textbf{SPD\textdownarrow} & \textbf{KPA\textuparrow} & \textbf{TC\textuparrow} & \phantom{} & \textbf{SPD\textdownarrow} & \textbf{KPA\textuparrow} & \textbf{TC\textuparrow}\\
\toprule
&\multicolumn{6}{c}{\textbf{2-Shot In-Context Learning}}\\
\midrule
VELMA-GPT3      & 26.0   & 39.6  & 6.2  &&  21.3 & 46.2   &   7.5  \\
\bullet \text{VELMA-GPT3}   & 27.5   &  24.8  &  3.0  && 23.7   &  28.5  &  3.5   \\
\text{VELMA-GPT3 (w/ NPE-CoT) }         & 27.2 \scriptsize{(\textcolor{red}{\textdownarrow 1.09\%})}   &  31.2 \scriptsize{(\textcolor{blue}{\textuparrow 25.81\%})}  &  4.5 \scriptsize{(\textcolor{blue}{\textuparrow 50.00\%})}  && 23.5 \scriptsize{(\textcolor{red}{\textdownarrow 0.84\%})}  &  34.5 \scriptsize{(\textcolor{blue}{\textuparrow 21.05\%})}  &  5.3 \scriptsize{(\textcolor{blue}{\textuparrow 51.43\%})}   \\
\text{VELMA-GPT3 (w/ NPE-PS) }         & 27.0 \scriptsize{(\textcolor{red}{\textdownarrow 1.82\%})}   &  32.0 \scriptsize{(\textcolor{blue}{\textuparrow 29.03\%})}  &  4.5 \scriptsize{(\textcolor{blue}{\textuparrow 50.00\%})}  && 23.6 \scriptsize{(\textcolor{red}{\textdownarrow 0.42\%})}  &  32.4 \scriptsize{(\textcolor{blue}{\textuparrow 13.86\%})}  &  4.3 \scriptsize{(\textcolor{blue}{\textuparrow 22.86\%})}   \\
\text{VELMA-GPT3 (w/ NPE-RP) }         & 26.4 \scriptsize{(\textcolor{red}{\textdownarrow 4.00\%})}   &  33.1 \scriptsize{(\textcolor{blue}{\textuparrow 33.47\%})}  &  5.0 \scriptsize{(\textcolor{blue}{\textuparrow 66.67\%})}  && 23.5 \scriptsize{(\textcolor{red}{\textdownarrow 0.84\%})}  &  30.3 \scriptsize{(\textcolor{blue}{\textuparrow 6.32\%})}  &  4.0 \scriptsize{(\textcolor{blue}{\textuparrow 14.29\%})}   \\

\midrule
VELMA-LLaMa2     & 43.0  &  36.9  &  1.9  & & 36.7  &  43.2  &  2.6   \\
\circ \text{VELMA-LLaMa2}   & 45.0 &  15.6   &  0.5  & & 42.0   &  15.4   &  0.9  \\

\text{VELMA-LLaMa2 (w/ NPE-CoT) }         & 43.4 \scriptsize{(\textcolor{red}{\textdownarrow 3.56\%})}  &  17.2 \scriptsize{(\textcolor{blue}{\textuparrow 10.26\%})}  &  0.7 \scriptsize{(\textcolor{blue}{\textuparrow 40.00\%})}  & & 41.2 \scriptsize{(\textcolor{red}{\textdownarrow 1.90\%})}  &  19.8 \scriptsize{(\textcolor{blue}{\textuparrow 28.57\%})}  &  1.0 \scriptsize{(\textcolor{blue}{\textuparrow 11.11\%})}   \\

\text{VELMA-LLaMa2 (w/ NPE-PS) }         & 43.9 \scriptsize{(\textcolor{red}{\textdownarrow 2.44\%})}  &  18.1 \scriptsize{(\textcolor{blue}{\textuparrow 16.03\%})}  &  0.8 \scriptsize{(\textcolor{blue}{\textuparrow 60.00\%})}  & & 40.0 \scriptsize{(\textcolor{red}{\textdownarrow 4.76\%})}  &  20.1 \scriptsize{(\textcolor{blue}{\textuparrow 30.52\%})}  &  1.0 \scriptsize{(\textcolor{blue}{\textuparrow 11.11\%})}   \\

\text{VELMA-LLaMa2 (w/ NPE-RP) }         & 43.2 \scriptsize{(\textcolor{red}{\textdownarrow 4.00\%})}  &  16.9 \scriptsize{(\textcolor{blue}{\textuparrow 8.33\%})}  &  0.6 \scriptsize{(\textcolor{blue}{\textuparrow 20.00\%})}  & & 41.0 \scriptsize{(\textcolor{red}{\textdownarrow 2.38\%})}  &  21.1 \scriptsize{(\textcolor{blue}{\textuparrow 37.01\%})}  &  1.1 \scriptsize{(\textcolor{blue}{\textuparrow 22.22\%})}   \\



\midrule
&\multicolumn{6}{c}{\textbf{LLM Finetuning, full training set}}\\
\midrule
VELMA-RBL     & 15.6 & 55.1 & 24.5&& 9.1 &  70.2 &  42.5 \\
\circ \text{VELMA-RBL}   & 28.9  & 14.9  & 3.9  && 21.2 & 29.5  & 11.4  \\
\text{VELMA-RBL (w/ NPE-CoT)}   & 26.6 \scriptsize{(\textcolor{red}{\textdownarrow 7.96\%})}  &  25.5 \scriptsize{(\textcolor{blue}{\textuparrow 71.14\%})}  &  6.1 \scriptsize{(\textcolor{blue}{\textuparrow 56.41\%})}  & & 15.4 \scriptsize{(\textcolor{red}{\textdownarrow 27.36\%})}  &  52.2 \scriptsize{(\textcolor{blue}{\textuparrow 76.95\%})}  &  17.1 \scriptsize{(\textcolor{blue}{\textuparrow 50.00\%})}   \\

\text{VELMA-RBL (w/ NPE-PS) }      & 28.5 \scriptsize{(\textcolor{red}{\textdownarrow 1.38\%})}  &  23.3 \scriptsize{(\textcolor{blue}{\textuparrow 56.38\%})}  &  5.5 \scriptsize{(\textcolor{blue}{\textuparrow 41.03\%})}  & & 16.7 \scriptsize{(\textcolor{red}{\textdownarrow 21.22\%})}  &  53.1 \scriptsize{(\textcolor{blue}{\textuparrow 80.00\%})}  &  16.5 \scriptsize{(\textcolor{blue}{\textuparrow 44.74\%})}   \\

\text{VELMA-RBL (w/ NPE-RP)}   & 25.1 \scriptsize{(\textcolor{red}{\textdownarrow 13.15\%})}  &  32.0 \scriptsize{(\textcolor{blue}{\textuparrow 114.77\%})}  &  12.8 \scriptsize{(\textcolor{blue}{\textuparrow 228.21\%})}  & & 10.7 \scriptsize{(\textcolor{red}{\textdownarrow 49.53\%})}  &  65.1 \scriptsize{(\textcolor{blue}{\textuparrow 120.68\%})}  &  29.0 \scriptsize{(\textcolor{blue}{\textuparrow 154.39\%})}   \\
\bottomrule
\end{tabular}
}
\label{tab:res_defence}
\end{table*}

==> tables/supp_table_FT.tex <==
\begin{table*}[h]
\centering
\caption{Results for the VELMA model with various LLM models using three Navigational Prompt Engineering (NPE) Defense strategies after the Navigational Prompt Suffix (NPS) Attack on the Touchdown and Map2seq datasets in an unseen scenario. $\circ$ and $\bullet$ indicate white-box and black-box attacks, respectively, by applying the NPS Attack to the LLaMa model. NPE-Cot denotes NPE with Chain of Thought prompting, NPE-PS denotes NPE with Plan-and-Solve prompting, and NPE-RP denotes NPE with Role-Play prompting.
}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
&\multicolumn{3}{c}{\textbf{Touchdown}} & \phantom{} &\multicolumn{3}{c}{\textbf{Map2seq}} \\ 
\cmidrule{2-4} \cmidrule{6-8} 
    \textbf{LLM Models} & \textbf{SPD\textdownarrow} & \textbf{KPA\textuparrow} & \textbf{TC\textuparrow} & \phantom{} & \textbf{SPD\textdownarrow} & \textbf{KPA\textuparrow} & \textbf{TC\textuparrow}\\
\toprule
&\multicolumn{6}{c}{\textbf{LLM Finetuning, full training set}}\\
\midrule

VELMA-FT     & 18.8  &  53.2  &  21.2  & & 9.6  &  68.5  &  38.5   \\
\text{VELMA-FT} \dagger  & 29.5 &  29.9   &  8.0  & & 34.5   &  24.2   &  3.8  \\

\text{VELMA-FT (w/ NPE-CoT) }         & 24.6 \scriptsize{(\textcolor{red}{\textdownarrow 16.61\%})}  &  31.2 \scriptsize{(\textcolor{blue}{\textuparrow 4.35\%})}  &  10.4 \scriptsize{(\textcolor{blue}{\textuparrow 30.00\%})}  & & 34.4 \scriptsize{(\textcolor{red}{\textdownarrow 0.29\%})}  &  25.8 \scriptsize{(\textcolor{blue}{\textuparrow 6.61\%})}  &  6.3 \scriptsize{(\textcolor{blue}{\textuparrow 65.79\%})}   \\

\text{VELMA-FT (w/ NPE-PS) }         & 25.1 \scriptsize{(\textcolor{red}{\textdownarrow 14.92\%})}  &  30.3 \scriptsize{(\textcolor{blue}{\textuparrow 1.34\%})}  &  9.1 \scriptsize{(\textcolor{blue}{\textuparrow 13.75\%})}  & & 30.2 \scriptsize{(\textcolor{red}{\textdownarrow 12.46\%})}  &  32.8 \scriptsize{(\textcolor{blue}{\textuparrow 35.54\%})}  &  9.3 \scriptsize{(\textcolor{blue}{\textuparrow 144.74\%})}   \\

\text{VELMA-FT (w/ NPE-RP) }         & 25.3 \scriptsize{(\textcolor{red}{\textdownarrow 14.24\%})}  &  34.4 \scriptsize{(\textcolor{blue}{\textuparrow 15.05\%})}  &  12.9 \scriptsize{(\textcolor{blue}{\textuparrow 61.25\%})}  & & 16.1 \scriptsize{(\textcolor{red}{\textdownarrow 53.33\%})}  &  54.5 \scriptsize{(\textcolor{blue}{\textuparrow 125.21\%})}  &  21.4 \scriptsize{(\textcolor{blue}{\textuparrow 463.16\%})}   \\





\bottomrule
\end{tabular}
}
\label{tab:res_defence}
\end{table*}

==> tables/supp_table_Llama.tex <==
\begin{table*}[h]
\centering
\caption{Results for the VELMA model with various LLM models using three Navigational Prompt Engineering (NPE) Defense strategies after the Navigational Prompt Suffix (NPS) Attack on the Touchdown and Map2seq datasets in an unseen scenario. $\circ$ and $\bullet$ indicate white-box and black-box attacks, respectively, by applying the NPS Attack to the LLaMa model. NPE-Cot denotes NPE with Chain of Thought prompting, NPE-PS denotes NPE with Plan-and-Solve prompting, and NPE-RP denotes NPE with Role-Play prompting.
}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
&\multicolumn{3}{c}{\textbf{Touchdown}} & \phantom{} &\multicolumn{3}{c}{\textbf{Map2seq}} \\ 
\cmidrule{2-4} \cmidrule{6-8} 
    \textbf{LLM Models} & \textbf{SPD\textdownarrow} & \textbf{KPA\textuparrow} & \textbf{TC\textuparrow} & \phantom{} & \textbf{SPD\textdownarrow} & \textbf{KPA\textuparrow} & \textbf{TC\textuparrow}\\
\toprule
&\multicolumn{6}{c}{\textbf{2-Shot In-Context Learning}}\\
\midrule

VELMA-LLaMa1     & 36.7  &  37.5  &  1.1  & & 35.4  &  30.0  &  1.0   \\
\text{VELMA-LLaMa1}\dagger   & 38.4 &  13.8   &  0.4  & & 39.9   &  16.7   &  0.1  \\

\text{VELMA-LLaMa1 (w/ NPE-CoT) }         & 37.0 \scriptsize{(\textcolor{red}{\textdownarrow 3.65\%})}  &  14.5 \scriptsize{(\textcolor{blue}{\textuparrow 5.07\%})}  &  0.5 \scriptsize{(\textcolor{blue}{\textuparrow 25.00\%})}  & & 38.8 \scriptsize{(\textcolor{red}{\textdownarrow 2.76\%})}  &  18.7 \scriptsize{(\textcolor{blue}{\textuparrow 11.98\%})}  &  0.8 \scriptsize{(\textcolor{blue}{\textuparrow 700.00\%})}   \\

\text{VELMA-LLaMa1 (w/ NPE-PS) }         & 38.1 \scriptsize{(\textcolor{red}{\textdownarrow 0.78\%})}  &  14.4 \scriptsize{(\textcolor{blue}{\textuparrow 4.35\%})}  &  0.4 \scriptsize{(\textcolor{blue}{\textuparrow 0.00\%})}  & & 38.7 \scriptsize{(\textcolor{red}{\textdownarrow 3.01\%})}  &  17.8 \scriptsize{(\textcolor{blue}{\textuparrow 6.59\%})}  &  0.3 \scriptsize{(\textcolor{blue}{\textuparrow 300.00\%})}   \\

\text{VELMA-LLaMa1 (w/ NPE-RP) }         & 37.5 \scriptsize{(\textcolor{red}{\textdownarrow 2.34\%})}  &  15.1 \scriptsize{(\textcolor{blue}{\textuparrow 9.42\%})}  &  0.5 \scriptsize{(\textcolor{blue}{\textuparrow 25.00\%})}  & & 39.0 \scriptsize{(\textcolor{red}{\textdownarrow 2.26\%})}  &  17.7 \scriptsize{(\textcolor{blue}{\textuparrow 5.99\%})}  &  0.4 \scriptsize{(\textcolor{blue}{\textuparrow 400.00\%})}   \\





\bottomrule
\end{tabular}
}
\label{tab:res_defence}
\end{table*}
